Theory of colloidal stabilization by unattached polymers

Stable colloidal dispersions with evenly distributed particles are important for many technological applications. Due to Brownian motion colloidal particles have constant collisions with each other which often lead to their aggregation driven by the long range van der Waals attraction. As a result the colloidal systems often tend to precipitate. A number of methods have been devised to minimize the effect of long-range van der Waals attraction between colloidal particles or to override the influence of the attraction in order to provide the colloidal stability.In the PhD thesis we investigated the colloidal stabilization in solutions of free polymers which is commonly referred to as depletion stabilization. Previous theoretical studies of free-polymer induced (FPI) stabilization were based on oversimplified models involving uncontrolled approximations. Even the most basic features of the depletion stabilization phenomenon were unknown. It was unclear how the PI repulsion depends on the solution parameters, polymer structure and monomer/surface interactions.The free polymer chains were modeled as random walks in a self-consistent molecular field that satisfied to diffusion-like integro-differential equation. As the molecular field we used the chemical potential that for semi-dilute polymer solution can be represented as a virial expansion where we took into account only second and third virial coefficients of the polymer solution. Varying the parameters like polymer stiffness, polymer length, polymer concentration and solvent regime (like theta solvent) whether it is for purely repulsive colloidal surface, adsorbed surface or surface with grafted polymer layer we were able to enhance the repulsive barrier due to the free polymers between the particles and therefore found conditions for kinetic stabilization of the system.

==> TitlePage/Logos/TitlePage.tex <==
\begin{titlepage}
\begin{center}

\textsc{\LARGE \href{https://www.unistra.fr} % Your university's URL
                {Université de Strasbourg}}\\[1.5cm] % University name
\textsc{\Large Doctoral Thesis}\\[0.5cm] % Thesis type

\HRule \\[0.4cm] % Horizontal line
{\huge \bfseries \ttitle}\\[0.4cm] % Thesis title
\HRule \\[1.5cm] % Horizontal line
 
\begin{minipage}{0.4\textwidth}
\begin{flushleft} \large
\emph{Author:}\\
\href{http://www.linkedin.com/pub/alexey-shvets/63/152/b02}{Alexey Shvets} % Author name - remove the \href bracket to remove the link
\end{flushleft}
\end{minipage}
\begin{minipage}{0.4\textwidth}
\begin{flushright} \large
\emph{Directeur de thèse:} \\
\href{http://www-ics.u-strasbg.fr/spip.php?article290}{Dr. Alexander Semenov} % Supervisor name - remove the \href bracket to remove the link  
\end{flushright}
\end{minipage}\\[2cm]
 
 
\large \textit{Thèse présentée pour obtenir le titre de Docteur de l’Université de Strasbourg\\ 
			   Discipline : Physique}\\[1.0cm] % University requirement text

\begin{minipage}{0.7\textwidth}
\begin{flushleft} 
\textit{Membres du Jury:}\\[0.4cm] 
\emph{Rapporteur externe:} 
\href{https://www.google.com}{A. Subbotin}\\
Institute of Petrochemical Synthesis, Russian Academy of Sciences, Moscow, Russia \\[0.4cm]
\emph{Rapporteur externe:} 
\href{http://www.personal.reading.ac.uk/~sms06al2/}{A. Likhtman}\\
Professor,  University of Reading, Reading, UK \\[0.4cm]
\emph{Examinateur interne:} 
\href{http://www-ics.u-strasbg.fr/spip.php?article128}{J. Baschnagel}\\
Professeur, Université de Strasbourg, Strasbourg, France \\[0.4cm]
%\emph{Examinateur externe:} 
%\href{http://www.phys.ufl.edu/~sergei/}{S. Obukhov}\\
%Professor, University of Florida, Gainesville, USA\\[0.4cm]
%\emph{Examinateur externe:} 
%\href{http://www.physics.nyu.edu/Grosberg/}{A. Grosberg}\\
%Professor, New York University, New York, USA
\end{flushleft}
\end{minipage}
\begin{minipage}{0.2\textwidth}
\begin{flushleft} 
\end{flushleft}
\end{minipage}\\[0.8cm]
\includegraphics[scale=0.1]{../TitlePage/Logos/strasbourg_logo.jpg} 
\includegraphics[scale=0.1]{../TitlePage/Logos/ics_logo.jpg} 
\includegraphics[scale=0.4]{../TitlePage/Logos/cnrs_logo.png} 
\includegraphics[scale=0.2]{../TitlePage/Logos/irtg_logo.png} \\
%\groupname\\\deptname\\[2cm] % Research group name and department name

 
{\large \today}\\[4cm] % Date
 
\vfill
\end{center}

\end{titlepage}
